Distributed Symmetric Key Establishment: a Scalable Quantum-Safe Key Distribution Protocol

Pre-shared keys (PSK) have been widely used in network security. Nonetheless, existing PSK solutions are not scalable. Moreover, whenever a new user joins a network, PSK requires an existing user to get a new key before they are able to communicate with the new user. The key issue is how to distribute the PSK between different users. Here, we solve this problem by proposing a new protocol called Distributed Symmetric Key Establishment (DSKE). DSKE has the advantage of being scalable. Unlike standard public key infrastructure (PKI) which relies on computational assumptions, DSKE provides information-theoretic security in a universally composable security framework. Specifically, we prove the security (correctness and confidentiality) and robustness of this protocol against a computationally unbounded adversary, who additionally may have fully compromised a bounded number of the intermediaries and can eavesdrop on all communication. DSKE also achieves distributed trust through secret sharing. We present several implementations of DSKE in real environments, such as providing client services to link encryptors, network encryptors, and mobile phones, as well as the implementation of intermediaries, called Security Hubs, and associated test data as evidence for its versatility. As DSKE is highly scalable in a network setting with no distance limit, it is expected to be a cost-effective quantum-safe cryptographic solution to the network security threat presented by quantum computers.

==> text/dske_protocol/dske_skeleton.tex <==
\section{Security of the DSKE protocol} 
\label{sec:dske_security}

\subsection{Cryptographic Primitives}\label{subsec:primitives}
\subsubsection{Message validation (authentication)}

The following \cref{thm:hash_function_correctness} is a consequence of the hashing scheme being a Carter--Wegman universal hash function family \cite{wegman1981new}. This polynomial function family is described by Bernstein \cite{Bernstein2007}.

\begin{theorem}\label{thm:hash_function_correctness} ~ \\
    Denote $\mbf{v} = (v_{1},...,v_{s})$ and $\mbf{v}^{*} = (v^{*}_{1},...,v^{*}_{s})$. \\
    Let $\Omega=F^2$ be a sample space with uniform probability. \\
    Let $h_{C,D}(\mbf{v})=D+\sum_{j=1}^{s}C^{j} v_{j}$ define a family of functions with random variables $(C,D)\in\Omega$ as selection parameters.
    Let $s\ne0$. Let $t\in F$ be given.
    Then, $\max_{t^{*},\mbf{v}^{*}\ne\mbf{v}} \Pr(t^{*}=h_{C,D}(\mbf{v}^{*})~|~t=h_{C,D}(\mbf{v})) = \min(\frac{s}{|F|},1)$.
\end{theorem}
\begin{proof}
	See \Cref{thm:message_correctness} in \Cref{app:hash_message}.
\end{proof}

Given a message $\mbf{v}$ together with a valid tag $t=h_{c,d}(\mbf{v})$ (with $(c,d)$ being described by the uniform random variables $C,D$), \cref{thm:hash_function_correctness} tells us that the maximal success probability for a forger to create a differing message $\mbf{v}^{*}$ and a new hash value $t^{*}$ such that these correspond (i.e., that $t^{*}=h_{C,D}(\mbf{v}^{*})$) is at most $\min(\frac{s}{|F|},1)$ when the message length $s$ is nonzero. This extends to $s=0$ due to the nonexistence of differing messages of that length.
In the other words, not knowing $(c,d)$ makes it highly improbable (for large $|F|$) for the forger to successfully substitute a tag and \textit{differing} message.

The theorem does not apply without a prior message. In the absence of a prior message, the probability that a forged message will be validated is $\frac{1}{|F|}$, which is independent of the length $s$.

\subsubsection{Secret Confidentiality and Validation}

Shamir introduced a secret sharing scheme that produces $n$ shares, any $k$ of which are sufficient to reconstruct the secret, but any $k-1$ of which give no information about the secret \cite{shamir1979share}. We state theorems here and leave proofs in \Cref{app:hash_secret}.

\begin{theorem}\label{thm:secret_confidentiality}
    In a Shamir secret sharing scheme with threshold $k$, the shared secret is independent of any subset of the shares of size $k-1$ or less.
\end{theorem}

\Cref{thm:secret_confidentiality} tells us that, under the constraint of access to only $k-1$ shares, a Shamir threshold-$(n,k)$ secret sharing scheme has perfectly secure confidentiality. 

\begin{theorem}\label{thm:secret_linearity}
    In a Shamir secret sharing scheme with threshold $k$, for any given set of $k$ shares, the secret is a linear combination of the shares.
\end{theorem}


\begin{theorem}\label{thm:hash_function_confidentiality}
    Denote $\mbf{Y}=(Y_{(1)},\dots,Y_{(m)})$. \\
    Let $\Omega=F^{3+m}$ be a sample space.
    Let $(C,D,E,\mbf{Y})\in\Omega$, with $D$ uniform and independent of $C,E$ and $\mbf{Y}$. \\
    Let $T=h'_{C,D,E}(\mbf{Y})=D+CE+\sum_{j=1}^{m}C^{j+1}Y_{(j)}$. \\
    Then $T$ is independent of $\mbf{Y}$.
\end{theorem}
Its proof is straightforward by using \Cref{lem:indepsum} in \Cref{app:hash_secret}. \Cref{thm:hash_function_confidentiality} tells us that no information is obtained from the tag ($o^A$ as $T$) about the secret ($S^A$ as $\mbf{Y}$).  Thus, given the perfectly secure confidentiality provided by a Shamir secret sharing scheme for up to $k-1$ shares being known, publishing the tag does not impact this confidentiality.

Given a Shamir secret sharing scheme, the resulting secret is malleable: a modification of any share will modify the reconstructed secret in a known way, in the same way that modifying the ciphertext of one-time-pad encryption modifies the decrypted plaintext.  Normally, a message authentication code would be employed to allow detection of such a change, but this needs a shared key to implement.  Transmitting a validation key via the same secret sharing scheme violates the normal premise for authentication: that the validation key is assured to be the same at both sides.  \Cref{thm:secret_validation} gives us a way to transmit such a key using the same (malleable) secret sharing scheme while providing authenticity, under the same premise that the secret sharing scheme already has.  We believe that this is a novel construction\footnote{A related objective is presented in \cite{ostrev2019composable}.}.

\begin{theorem}\label{thm:secret_validation}
    Denote $\mbf{y}=(y_{(1)},\dots,y_{(m)})$ and $\mbf{y}'=(y'_{(1)},\dots,y'_{(m)})$.
    Let $\Omega=F^3$ be a sample space with uniform probability.
    Let $h'_{C,D,E}(\mbf{y})=D+CE+\sum_{j=1}^{m}C^{j+1}y_{(j)}$ define a family of hash functions with random variables $(C,D,E)\in\Omega$ as selection parameters. Let $m\ne0.$
    Then, $\max_{t',c',d',e',\mbf{y}'\ne\mbf{y}} \Pr(t+t'=h'_{C+c',D+d',E+e'}(\mbf{y}+\mbf{y}')~|~t=h'_{C,D,E}(\mbf{y}))\le\min(\frac{m+1}{|F|},1)$.
\end{theorem}

\Cref{thm:secret_validation} gives us an upper bound on the probability of validating a secret with a nontrivial alteration, with three confidential uniform elements and the alteration constrained to \textit{addition} of a vector to $(C,D,E,\mbf{y})$. The premise for the theorem is assured by the secret sharing scheme. There are $n\choose k$ subsets of $k$ shares and hence reconstructions, but a probability is upper-bounded at $1$, giving an upper bound on the probability of any of the ${n\choose k}$ reconstructed secret candidates passing the validation of $\epsilon\le\min({n\choose k}\frac{m+1}{|F|},1)$.

Combining \Cref{thm:secret_confidentiality,thm:secret_linearity,thm:hash_function_confidentiality,thm:secret_validation} leads to the following result:

The $(n,k)$-Shamir secret sharing scheme and a polynomial validation code for transmitting $3+m$ elements of the same finite field $F$, where the first 3 elements are uniform, of which the first $3$ are consumed as $u^A$ and the remaining $m$ elements are $S^A$, has
\begin{itemize}
    \setlength\itemsep{0em}
    \item $\epsilon$-secure correctness with $\epsilon\le\min({n\choose k}\frac{m+1}{|F|},1)$
    \item perfectly secure confidentiality
\end{itemize}
against a computationally unbounded adversary who can access and modify up to $k-1$ shares and block but not access or modify any of the remaining shares.

This leverages the secrecy provided by the sharing scheme to deliver the key used for secure validation of the secret that is simultaneously delivered.  This is novel in the sense that it ensures correctness (authentication) in addition to retaining the confidentially of the secret sharing scheme without imposing additional security requirements, i.e., it assumes only that no more than $k-1$ of the shares are compromised, as with the sharing scheme, whereas normally the key for validation would be assumed to be pre-shared.

\subsection{Threat Model}
\label{subsec:threat_model}

A collection of adversarial entities can include a coalition of end users other than Alice and Bob, eavesdroppers, and a subset of the Security Hubs. A compromised Security Hub may deviate from the protocol. No limits are placed on compromised hubs, but they cannot access or modify any confidential information held by other parties. This set of adversaries may collude to attempt to compromise the objective of the protocol between Alice and Bob. We call this collection of adversarial entities \textit{Eve}. 

As a robustness analysis of a protocol is concerned with an honest implementation of the protocol, which is a modified threat model from that of the correctness and confidentiality (i.e. \Cref{subsec:ideal_system}) analysis, we call Eve's behaviour \textit{passive Eve}: Eve is passive on all communication links, that is, she is allowed to listen to all the communications except for the initial sharing of tables by honest Security Hubs but she does not tamper; she is still given the ability to fully control compromised Security Hubs. When Eve is passive, we show that the DSKE protocol completes (i.e., does not abort) with a high probability.

\subsection{Assumptions}
\label{subsec:assumptions}

We list assumptions used in our security proof:
\begin{enumerate}[label = \roman*)]
    \item The pre-shared random data (PSRD) are securely delivered by all uncompromised Security Hubs to both Alice and Bob. By \textit{securely delivered}, we mean ensured confidentiality, integrity and proper identity verification through secure channels between Security Hubs and clients.\footnote{PSRD can be delivered by physically shipping a secure data storage device or via QKD links.}.
    \item The two users, Alice and Bob, are both honest.
    \item A number of the Security Hubs might be compromised, and this number has a known upper bound. 
    \item For the robustness analysis, a number of the involved Security Hubs might malfunction, either due to unavailability, communication failure\footnote{This type of malfunction includes the a communication link providing an incorrect sender identity to the receiver.}, or compromise, and this number has a known upper bound. This is incorporated with the assumption that Eve is passive on the communication links.
\end{enumerate}

\subsection{Composable Security in Constructive Cryptography}

As a cryptographic protocol is often combined with many other protocols, it is important to prove the security of the protocol in a composable security framework. The composability result in such a framework asserts that in analyzing the security of a complex protocol, one can simply decompose it into various subprotocols and analyze the security of each. Provided that each real subsystem constructed by a subprotocol is close to an ideal subsystem within some $\epsilon$, which is quantified by some distance measure (a pseudo-metric in abstract cryptography), the real system constructed from the combined protocol will then be close to the combined ideal system. The sum of the $\epsilon$-values for the subprotocols gives an $\epsilon$-value for the combined protocol.

The abstract cryptography framework \cite{MaurerRenner2011} uses a top-down approach. In this framework, one states the definitions and proves the security from the highest possible level of abstraction and proceeds downwards. When one deals with a specific instantiation of an abstract system in a lower level, as long as the lower level system satisfies the properties required in the higher-level proof, the composed protocol is secure. The constructive cryptography \cite{Maurer2011} is an application of the abstract cryptography framework to defining classical cryptographic primitives in a constructive way. In this framework, one specifies the resources that are used by a protocol, their required properties and some desired functionalities of an ideal system. If a protocol constructs the ideal system from the given resources, then it is secure. A secure protocol in this sense achieves the universally composable security. We briefly review the composable security definition in the constructive cryptography framework below and refer to \cite{Maurer2011} for further details.
\begin{definition}\label{def:composable_security}
    Let $\mf{R}$ and $\mf{S}$ be resources with the interface label set $\mc{I} =\{A, B, E\}$. Let $d$ be a pseudo-metric. We say that a protocol $\pi = (\pi^A, \pi^B)$ securely constructs $\mf{S}$ out of $\mf{R}$ within $\epsilon$ if the following conditions hold:
    \begin{enumerate}[label=(\roman*)]
        \item For converters $\alpha^E$ and $\gamma^E$ that emulate an honest behaviour at the $E$-interface of each system and block any distinguisher from the access of $E$-interface of each system,%
        \begin{aeq}
            d(\pi\mf{R}\alpha^E, \mf{S}\gamma^E) \leq \epsilon.
        \end{aeq}
        \item There exists a converter $\sigma^E$ such that%
        \begin{aeq}
            d(\pi \mf{R}, \mf{S}\sigma^E) \leq \epsilon.
        \end{aeq}%
    \end{enumerate}
    We use the construction notation $\mf{R} \xrightarrow{(\pi, \epsilon)} \mf{S}$ for this case.
\end{definition}

To prove the security of the DSKE protocol, we first show the security of a variant of the DSKE protocol, which we call the \textit{skeleton} DSKE protocol. It differs from the general DSKE protocol (which we presented in \Cref{sec:dske}) only by the assumption that channel authentication is perfectly secure, where a perfectly secure authentication scheme is defined as an $\epsilon$-secure authentication scheme for which $\epsilon = 0$. We call this an authenticated channel. In an authenticated channel, an adversary may be free to eavesdrop on the communication and to tamper with a message, but the receiver will detect with certainty whether the message has been altered. This may also be thought of as the limiting behaviour as the size of a message authentication code increases.

We analyze the security of the skeleton DSKE protocol in the framework of constructive cryptography. (Further details about the constructive cryptography can be found in \cite{Maurer2011}. Also see \cite{Portmann2022}.) After proving the security of the skeleton protocol, it is then straightforward to use the composability theorem \cite[Theorem 1]{Maurer2011} to prove the security of the general DSKE protocol. 





\subsubsection{Security}
\begin{figure*}[t]
    \includegraphics[width=\linewidth]{./figs/real.png}
    \caption{A real key distribution resource using $n$ Security Hubs. Each green box represents an authenticated channel labelled by $\mbf{A}^+$ with a suitable subscript that identifies the communicating parties. The secret key resource $\mbf{K}_{AP_i}$ is used to encrypt $Y_i$ and $\mbf{K}_{P_iB}$ is used to encrypt $\overline{Y}_i$. If a Hub $P_i$ is compromised, Eve determines values of $Y_i, T_i, \overline{Y}_i, \overline{T}_i$ by accepting $(\overline{Y}^E_i, \overline{T}^E_i)$ at the $E$-interface; the system outputs $(Y^E_i, T^E_i):=(Y_i, T_i)$ at the $E$-interface. For honest Hubs, since the ciphertext of $Y_i$ ($\overline{Y}_i$) reveals no information about $Y_i$ ($\overline{Y}_i$), we simply set $Y^E_i:={\perp}$ to indicate this. For each Hub $P_i$, a two-bit variable $Z^E_i$ as an input to the $E_i$-interface is used to set the behaviours of two relevant authenticated channels. The $E$-interface of the system consists of $E_1$, \dots, $E_n$, where the alphabets for those inputs and outputs are determined by the operation mode of each corresponding Hub. The operation mode of each Hub is predetermined and cannot be altered through the $E$-interface. Figure legend: ENC: encryption operation, DEC: decryption operation, SHARE-GEN: share generation, SEC-REC: secret reconstruction, SEC-VAL: secret validation.}
    \label{figs:real_protocol}
\end{figure*}

\begin{figure*}[t]
\centering
	\includegraphics[width=0.9\linewidth]{./figs/ideal_simulator.png}
	\caption{An ideal key agreement resource using $n$ Security Hubs with the simulator $\sigma^E$. Hubs are reordered for drawing purposes only. The set of compromised Hubs is denoted by $C$. The simulator $\sigma^E$ sets operation modes of the Security Hubs contained inside the ideal resource system. For Hubs in the set $C$, it sets the Hub $P_i$ to operate in the compromised mode and uses $Z^E_i:=00$ it receives from its $E$-interface to set the behaviours of two authenticated channels for the Hub $P_i$. For all other Hubs that are not in the set $C$, the simulator $\sigma^E$ sets the Hub $P_j$ to operate in the honest mode and uses $Z^E_j \in \{00, 01, 10, 11\}$ to set the behaviours of two authenticated channels for the Hub $P_j$. The $E$-interface of the simulator also accepts the a pair of values $(\overline{Y}^E_i,\overline{T}^E_i)$ and it outputs $(Y^E_i, T^E_i)$ received from the ideal system. The allowed alphabets for those variables are determined by the operation mode of each corresponding Hub.}
	\label{figs:ideal+simulator}
\end{figure*}

We first discuss the security of the skeleton DSKE protocol. In the constructive cryptography framework, one needs to show the real resource combined with the protocol is close to the ideal resource that achieves the desired functionalities. We leave the detailed description of the relevant ideal system, real system, converter, distinguisher and simulator in \Cref{app:composable_security}. \Cref{figs:real_protocol} provides a schematic description of the real system and \Cref{figs:ideal+simulator} shows an example of a simulator with the ideal system.  We present the main theorems and discuss the proof ideas here. All technical details will be presented in \Cref{app:composable_security}.
\begin{theorem}\label{thm:skeleton_security}
	Under the assumptions listed in \Cref{subsec:assumptions}, the protocol $\pi^s = (\pi^A, \pi^B)$ described above (depicted in \Cref{figs:real_protocol}) is $\epsilon$-secure, where $\epsilon=\min({n \choose k}\frac{m+1}{|F|},1)$, which is determined by the family of hash functions used in the protocol as described in \cref{thm:secret_validation} as well as the choices of $n$ and $k$ in the $(n, k)$-threshold scheme. 
\end{theorem}


 To prove the security, we need to check two conditions in the composable security definition (see \Cref{def:composable_security}). The first condition is concerned with the situation where the $E$-interface is not accessible by the distinguisher. In this situation, the real system is completely characterized by the probability distribution $P_{S^A,S^B}$ and the ideal system with the simulator $\sigma^E$ is completely characterized by the probability distribution $Q_{S^A,S^B}$. The distinguishing advantage is the statistical distance between $P_{S^A,S^B}$ and $Q_{S^A,S^B}$. It is straightforward to compute this using properties of the secret-authenticating tag and the assumption that at most $k-1$ Hubs are compromised. The second condition deals with the situation where the ideal system is attached to the simulator $\sigma_E$ discussed previously, which is shown in \Cref{figs:ideal+simulator}. As the real system (as shown in \Cref{figs:real_protocol}) is completely characterized by $P_{S^A,S^B,(Y^E_i,T^E_i,\overline{Y}^E_i,\overline{T}^E_i, Z^E_i)_i}$ and the ideal system with the simulator $\sigma^E$ is completely characterized by $Q_{S^A,S^B,(Y^E_i,T^E_i,\overline{Y}^E_i,\overline{T}^E_i, Z^E_i)_i}$, our task is to compute statistical distance between $P_{S^A,S^B,(Y^E_i,T^E_i,\overline{Y}^E_i,\overline{T}^E_i, Z^E_i)_i}$ and $Q_{S^A,S^B,(Y^E_i,T^E_i,\overline{Y}^E_i,\overline{T}^E_i, Z^E_i)_i}$. It follows a similar procedure in this case with an additional observation: it is unfavorable for the adversary to disrupt the authenticated channels as doing so can only make two systems more indistinguishable.


The security of the general DSKE protocol follows straightfowardly from \Cref{thm:skeleton_security} and the composability theorem \cite[Theorem 1]{Maurer2011}. Let $\mf{R}_g$ denote the resource used in the general DSKE protocol which differs from the resource used in the skeleton DSKE protocol in the following way: replacing each authenticated channel by an insecure channel and a secret key resource. 

\begin{theorem}
    ~\\The protocol $\pi^g = (\pi^s, \pi^{\auth}_{AP_1}, \dots, \pi^{\auth}_{AP_n}, \pi^{\auth}_{P_1B}, \dots \pi^{\auth}_{P_nB})$ securely constructs the ideal resource $\mf{S}$ out of the resource $\mf{R}_g$ within $\epsilon + 2n \epsilon'$, where each of $\pi^{\auth}_{AP_i}$ and $\pi^{\auth}_{P_iB}$ securely construct authenticated channels $\mbf{A}^+_{AP_i}$, $\mbf{A}^+_{P_iB}$ within $\epsilon'$, respectively, where $\epsilon = \min({n \choose k}\frac{m+1}{|F|}, 1)$ and $\epsilon' = \min(\frac{s}{|F|},1)$. 
\end{theorem}

\subsubsection{Robustness}\label{subsec:skeleton_robustness}

Robustness of a protocol is the condition that the protocol does not abort when Eve is passive (restricted to modifying the messages of compromised Hubs only), as defined in \Cref{subsec:threat_model}.  We say a protocol is $\epsilon$-robust if its aborting probability is at most $\epsilon$ in the case of this restriction. 
When restricted in this way, the aborting probability for the skeleton DSKE protocol is at most $\epsilon=\min({n \choose k}\frac{m+1}{|F|},1)$ when the number of honest Security Hubs is at least $k$ and the number of compromised Security Hubs is at most $k-1$.\footnote{The second condition becomes significant when $2k\le n$, due to multiple competing reconstructed secrets.}
\begin{theorem}[Robustness of a skeleton DSKE protocol]\label{thm:robustness_skeleton}
	Under the assumptions listed in \Cref{subsec:assumptions}, when the upper bound on the number of compromised Security Hubs is no greater than $\min(n-k, k-1)$, the skeleton DSKE protocol is $\epsilon$-robust with $\epsilon = \min({n \choose k} \frac{m+1}{|F|}, 1)$.
\end{theorem}
We omit this proof here as it is straightforward to show using the secret validation step of the protocol and the properties of secret-authenticating tag. We present a complete proof in \Cref{app:composable_security}.
%\begin{proof}
%	When Eve is passive, all authenticated channels in the skeleton DSKE protocol faithfully transmit messages. We note that a message using a fake identity gets rejected by the receiver without consuming any secret key resources by the assumption that a communication link provides the originating identity to the receiver. In other words, Eve cannot impersonate an honest Security Hub by using compromised Hubs to mount an attack to exhaust data in a table shared by a Security Hub and a user.
 
 %   If the number of honest Security Hubs is at least $k$ (which means the number of compromised Hubs cannot be more than $n-k$) and the number of compromised Hubs is at most $k-1$, the only condition that causes Bob to abort is when there are multiple different candidate tuples $(u^A, s^A, o^A)$ that pass the secret validation step. That is, in addition to the correct secret reconstructed using shares from $k$ honest Security Hubs, there must exist at least one different secret candidate that also passes the secret validation step. For each possible guess of the $(u^A, s^A)$ other than the correct secret, it can pass the secret validation step with a probability at most $\min(\frac{m+1}{|F|},1)$ due to \cref{thm:secret_validation}. Since there are at most ${n \choose k}$ valid candidates to go through the secret validation step, the aborting probability in this case is at most $\min({n \choose k}\frac{m+1}{|F|},1)=: \epsilon$. Thus, the skeleton DSKE protocol is $\epsilon$-robust when the upper bound on the number of compromised Security Hubs is no greater than $\min(n-k, k-1)$.
%\end{proof}
We note that passive Eve behaves in the same way for either an authenticated channel or an authentication protocol with an insecure channel. The $\epsilon$-robustness of the general DSKE protocol follows trivially from the $\epsilon$-robustness of the skeleton DSKE protocol.
\begin{theorem}[Robustness of a general DSKE protocol]\label{thm:robustness_general}
    When the upper bound on the number of compromised Security Hubs is no greater than $\min(n-k, k-1)$, a general DSKE protocol is $\epsilon$-robust with $\epsilon = \min({n \choose k} \frac{m+1}{|F|}, 1)$.
\end{theorem}


==> text/removed/deleted.tex <==
\subsection{Mathematical fundamentals}

\begin{enumerate}[leftmargin=0cm]

    \item[] \textbf{Fields:} Let $F=\mathrm{GF}(p^{r})$, a Galois field with $p$ a prime number and $r>0$ an integer. $F$ is a finite field with $|F|=p^{r}$ elements. Multiplication by a nonzero element of $F$ is a bijective mapping $F\to F$.

    \item[] \textbf{Addition of vectors:} The additive group of the vectors of dimension $m$ over $\mathrm{GF}(p^{r})$, namely $\mathrm{GF}(p^{r})^m$, is the same as the additive group of $\mathrm{GF}(p)^{rm}$.  This allows addition of vectors of suitable lengths over different fields to be compatible (i.e., to be the same group), when both fields have the same characteristic $p$.  For example, we can use this to match a Shamir secret sharing scheme of vectors over $\mathrm{GF}(2^{8})$, with a hash function over the field $\mathrm{GF}(2^{128})$ using bit-wise exclusive-or as addition while maintaining the properties that depend on this addition.  For simplicity of exposition, we use the same field for both the secret sharing scheme and the validating hash function.

    \item[] \textbf{Probability theory:}

    For any proposition $\prop(X, Y)$ of random variables $X$ and $Y$,%
    \begin{aeq}\label{eq:prob_prop}
        & \Pr(\prop(X, Y)) \\
        & = \sum_{y\in F} \Pr(\prop(X, Y) | Y = y) \Pr(Y = y).
    \end{aeq}

    When summing over all values of a random variable $Y \in \Omega$, where $\Omega$ is the relevant sample space for $Y$,%
    \begin{aeq}\label{eq:prob_sum_to_one}
        \sum_{y \in \Omega} \Pr(Y = y) = 1. 	
    \end{aeq}%
    When $X,Y\in \Omega$ are mutually independent and $X$ uniform,%
    \begin{aeq}\label{eq:prob_uniform}
        \Pr(X = x | Y = y) = 1/|\Omega|. 	
    \end{aeq}%
    Random variables $X$ and $Y$ are mutually independent if%
    \begin{aeq}\label{eq:prob_independent}
        \forall (x, y): & \Pr( (X, Y) = (x, y) ) \\
        & = \Pr( X = x ) \Pr( Y = y ). 	
    \end{aeq}

    \item[] \textbf{Statistical distance:} For two probability distributions $P_X$ and $Q_X$ of a random variable $X$ that can take any value in some set $\mathcal{X}$, the statistical or total variation distance between $P_X$ and $Q_X$ has the following properties:%
    \begin{aeq}\label{eq:statistical_distance_property}
        &\frac{1}{2}\sum_{x \in \mathcal{X}}|P_X(x)-Q_X(x)| \\
         = &\max_{\mathcal{X}':\mathcal{X}'\subseteq \mathcal{X}}\sum_{x \in \mathcal{X}'}(P_X(x)-Q_X(x)) \\
         = &\sum_{x: P_X(x) \geq Q_X(x)} (P_X(x)-Q_X(x)).
    \end{aeq}

\end{enumerate}

\begin{theorem}[{\cite[Theorem 1]{Maurer2011}}]\label{thm:composability}
	The security definition in \cref{def:composable_security} is generally composable if the pseudo-metric $d$ is compatible with the cryptographic algebra\footnote{We refer to \cite{Maurer2011} for the definitions of cryptographic algebra and compatibility of the pseudo-metric with cryptographic algebra. The pseudo-metric used in this paper is compatible with the underlying cryptographic algebra since we consider information-theoretic security so that if a distinguisher in the set of all distinguishers $\mathbb{D}$ is composed with another arbitrary system, it is still in $\mathbb{D}$. To avoid further distraction, we omit this definition here.}. The following statements hold:
	\begin{enumerate}[label=(\roman*)]
		\item If a protocol $\pi$ securely constructs a system $\mf{S}$ out of a system $\mf{R}$ within $\epsilon$ and another protocol $\pi'$ securely constructs a system $\mf{T}$ out of a system $\mf{S}$ within $\epsilon'$, then the serial composition $\pi\pi'$(running the protocol $\pi'$ after the protocol $\pi$) securely constructs the system $\mf{T}$ out of the system $\mf{R}$ within $\epsilon+\epsilon'$, i.e.,%
        \begin{aeq}
			& (\mf{R} \xrightarrow{(\pi, \epsilon)} \mf{S}) \;\land\; (\mf{S} \xrightarrow{(\pi', \epsilon')} \mf{T}) \\
            \implies & \mf{R} \xrightarrow{(\pi\pi', \epsilon+\epsilon')} \mf{T};
		\end{aeq}%
		\item If a protocol $\pi$ securely constructs a system $\mf{S}$ out of a system $\mf{R}$ within $\epsilon$ and another protocol $\pi'$ securely constructs a system $\mf{S}'$ out of a system $\mf{R}'$ within $\epsilon'$, then the parallel composition $\pi \parallel \pi'$ securely constructs the system $\mf{S} \parallel \mf{S}'$ out of the system $\mf{R} \parallel \mf{R}'$ within $\epsilon+\epsilon'$, i.e.,%
        \begin{aeq}
			& (\mf{R} \xrightarrow{(\pi, \epsilon)} \mf{S}) \;\land\; (\mf{R}' \xrightarrow{(\pi', \epsilon')} \mf{S}') \\
            \implies & \mf{R}\parallel\mf{R}' \xrightarrow{(\pi\parallel\pi', \epsilon+\epsilon')} \mf{S} \parallel \mf{S}';
        \end{aeq}%
        \item When a trivial converter, which applies the identity transformation to the resource that it connects to, is applied to a system $\mf{R}$, it perfectly constructs the system $\mf{R}$ out of itself, i.e.,%
        \begin{aeq}
            \mf{R} \xrightarrow{(\mathbf{1}, 0)} \mf{R},
        \end{aeq}%
        where $\mathbf{1}$ denotes the trivial converter.
	\end{enumerate}
\end{theorem}

\begin{remark}
    The first condition in \cref{def:composable_security} captures the correctness of the protocol when no adversary is present. In this case, the adversarial controls covered by $\alpha^E$ and $\gamma^E$ are not accessible to the distinguisher. The second condition captures the situation when an adversary is present. In that case, the converters $\alpha^E$ and $\gamma^E$ are removed so that the distinguisher has full access to Eve's interfaces, which are the $E$-interface in the real system, and the $E$-interface of a simulator $\sigma^E$ that is attached to the ideal system. 
\end{remark}

\subsubsection{Composability theorem}

\begin{figure}[ht]
    \includegraphics[width=\linewidth]{./figs/distinguisher.png}
    \caption{\label{figs:distinguisher}The distinguisher $\mf{D}$ connects to an unknown system, interacts with it and reproduces a one-bit output that indicates its guess about the identity of the unknown system.}
\end{figure}

\begin{proof}
    When Eve is passive, a general DSKE protocol behaves in the same way as its corresponding skeleton protocol. The reason is as follows. A general DSKE and its corresponding skeleton protocol differ in the availability of authenticated channels. In the general DSKE protocol, an authentication protocol constructs an authenticated channel out of a secret key resource and an insecure channel, while in the skeleton protocol, authenticated channels are assumed to be available. When Eve is passive, she does not tamper each communication channel. Each authenticated channel in the skeleton protocol and each channel constructed by the authentication protocol in the general protocol both faithfully transmit messages. Thus, the result of \cref{thm:robustness_skeleton} directly applies.
\end{proof}

\begin{figure}[t]
	\includegraphics[width=\linewidth]{./figs/local_distributors.png}
        \caption{Schematic of the Security Hub, showing the Security Server and the Local Distributors. The Security Server is responsible for managing PSRD duplicates with all Clients linked to the Hub, and the Local Distributor distributes PSRD to Clients in their geographical region. There are PSRD shipments between the Security Server and its Local Distributors so that both the Client and the Security Server can have matching matching tables. Upon delivering PSRD to Clients, the Local Distributor deletes its copy, so that only 2 copies are ever kept (in the Security Server and the Client).
        }
	\label{figs:securityhub}
\end{figure}

==> text/removed/dske_general.tex <==
% removed from main.tex

\section{Security of the general DSKE protocol}
\label{sec:dske_general}

To assist our discussion here, as shown in \Cref{figs:real_protocol}, we denote the secure key resource between Alice and the Hub $P_i$ as $\mbf{K}_{AP_i}$, the authenticated channel between Alice and the Hub $P_i$ as $\mbf{A}^{+}_{AP_i}$, the secure key resource between the Hub $P_i$ as $\mbf{K}_{P_iB}$, and the authenticated channel between the Hub $P_i$ and Bob as $\mathbf{A}^{+}_{P_iB}$. In the previous section, we have shown that $\pi^s$ securely constructs the ideal resource $\mf{S}$ out of $\mf{R}_s$ within $\epsilon$, where the real resource $\mf{R}_s$ in the skeleton DSKE protocol is defined as%
\begin{aeq}
	\mf{R}_s := & \mbf{K}_{AP_1} \parallel \mbf{A}^{+}_{AP_1} \parallel P_1 \parallel \mbf{K}_{P_1B} \parallel \mbf{A}^{+}_{P_1B}\parallel \dots \\
    & \parallel \mbf{K}_{AP_n} \parallel \mbf{A}^{+}_{AP_n} \parallel P_n \parallel\mbf{K}_{P_nB} \parallel \mbf{A}^{+}_{P_nB}.  
\end{aeq}%

The difference between a skeleton protocol and a general protocol using the same $(n, k)$-threshold scheme is the availability of authenticated channel resources. In a general DSKE protocol, we need to use a secure key resource and an insecure channel to construct an authenticated channel. An authentication protocol $\pi^{\auth}_{AP_i}$ (also $\pi^{\auth}_{P_iB}$) using a Carter--Wegman universal hash function family to produce message tags can securely construct an authenticated channel out of a secret key resource and an insecure channel within $\epsilon':=\min(\frac{s}{|F|},1)$ as shown in \Cref{thm:hash_function_correctness}. To distinguish this secret key resource from the secret key resource used in the skeleton protocol, we denote the new secret key resource by $\mbf{K}^{\auth}$ and the insecure channel by $\mbf{C}$ (with suitable subscripts). We then define the resource $\mf{R}_g$ used in the general DSKE protocol as%
\begin{aeq}
	\mf{R}_g :=& \; \mbf{K}_{AP_1} \parallel \mbf{K}^{\auth}_{AP_1} \parallel \mbf{C}_{AP_1} \parallel P_1 \\ & \parallel
    \mbf{K}_{P_1B} \parallel \mbf{K}^{\auth}_{P_1B} \parallel \mbf{C}_{P_1B}  \parallel \dots \\ & \parallel \mbf{K}_{AP_n} \parallel \mbf{K}^{\auth}_{AP_n} \parallel \mbf{C}_{AP_n} \parallel P_n \\ &\parallel \mbf{K}_{P_nB} \parallel \mbf{K}^{\auth}_{P_nB} \parallel \mbf{C}_{P_nB} . 
\end{aeq}%

Recall that $m$ is the length of the secret to be agreed and $s$ is the length of the message for which a tag is produced. We now show that the general DSKE protocol is $(\epsilon + 2n \epsilon')$-secure, where $\epsilon = \min({n \choose k}\frac{m+1}{|F|}, 1)$ and $\epsilon' = \min(\frac{s}{|F|},1)$.

\begin{theorem}
	The protocol $\pi^g = (\pi^s, \pi^{\auth}_{AP_1}, \dots, \pi^{\auth}_{AP_n}, \pi^{\auth}_{P_1B}, \dots \pi^{\auth}_{P_nB})$ securely constructs the ideal resource $\mf{S}$ out of the resource $\mf{R}_g$ within $\epsilon + 2n \epsilon'$, where each of $\pi^{\auth}_{AP_i}$ and $\pi^{\auth}_{P_iB}$ securely construct authenticated channels $\mbf{A}^+_{AP_i}$, $\mbf{A}^+_{P_iB}$ within $\epsilon'$, respectively, where $\epsilon = \min({n \choose k}\frac{m+1}{|F|}, 1)$ and $\epsilon' = \min(\frac{s}{|F|},1)$. 
\end{theorem}
\begin{proof}
	We start with showing the first condition in \cref{def:composable_security} where no adversary is present. We trivially have%
	\begin{aeq}
		\pi^{\auth}(\mbf{K}^{\auth}\parallel\mbf{C}) \alpha^E = \mbf{A}^{+} \beta^E
	\end{aeq}%
    for each choice of subscript ($AP_i$ or $P_iB$), where $\alpha^E$ and $\beta^E$ emulate an honest behaviour at Eve's interfaces, since both systems are equivalent to a channel that faithfully transmits a message between two parties (either $A$ and $P_i$ or $P_i$ and $B$). With a slight abuse of notation, we use $\alpha^{E^{2n}}$ and $\beta^{E^{2n}}$ to denote systems that emulate an honest behaviour at Eve's interfaces in $\pi^g\mf{R}_g$ and $\pi^s\mf{R}_s$, which include $2n$ authentication channels in the systems $\mf{R}_g$ and $\mf{R}_s$, respectively. We use $\gamma^{E^{2n}}$ to denote the system that emulates an honest behaviour at Eve's interfaces in $\mf{S}$. Thus,%
	\begin{aeq}
		& d(\pi^g \mf{R}_g \alpha^{E^{2n}}, \mf{S}\gamma^{E^{2n}}) \\
		\leq & d(\pi^g \mf{R}_g\alpha^{E^{2n}}, \pi^s \mf{R}_s \beta^{E^{2n}}) + d( \pi^s \mf{R}_s \beta^{E^{2n}}, \mf{S}\gamma^{E^{2n}})\\
		= &~ d( \pi^s \mf{R}_s \beta^{E^{2n}}, \mf{S}\gamma^{E^{2n}})	\leq \epsilon, 
	\end{aeq}%
    where the last inequality is shown in \cref{thm:skeleton_security}.
	
    We now analyze the case of an active adversary as required in the second condition in \cref{def:composable_security}. 
    As each of $\pi^{\auth}_{AP_i}$ and $\pi^{\auth}_{P_iB}$ securely construct authenticated channels $\mbf{A}^+_{AP_i}$, $\mbf{A}^+_{P_iB}$ within $\epsilon'$, respectively, there exist converters $\sigma^E_{AP_i}$ and $\sigma^E_{P_iB}$ such that%
    \begin{aeq}
        d(\pi^{\auth}_{AP_i}(\mbf{K}^{\auth}_{AP_i}\parallel\mbf{C}_{AP_i}), \mbf{A}_{AP_i}^+\sigma^E_{AP_i} ) \leq \epsilon',\\
        d(\pi^{\auth}_{P_iB}(\mbf{K}^{\auth}_{P_iB}\parallel\mbf{C}_{P_iB}), \mbf{A}_{P_iB}^+\sigma^E_{P_iB} ) \leq \epsilon'.
    \end{aeq}%
    We use $\sigma^{E}_{AP_iB}$ to denote  $\sigma^E_{AP_i} \parallel\sigma^E_{P_iB}$ and use $\sigma^{E^n}_{APB}$ to denote $n$-copies of $\sigma^{E}_{AP_iB}$ composed in parallel. For the ease of writing, we use a shorthand notation $\mbf{A}^{+}_{AP_iB}$ to denote $\mbf{A}^{+}_{AP_i} \parallel \mbf{A}^{+}_{P_iB}$ and use $\{\mbf{A}^{+}_{AP_iB}\}$ to denote $\mbf{A}^{+}_{AP_1B} \parallel \dots \parallel \mbf{A}^{+}_{AP_nB}$. Similarly, we use $\pi^{\auth}_{AP_iB}(\mbf{KC})$ to denote $\pi^{\auth}_{AP_i}(\mbf{K}^{\auth}_{AP_i} \parallel \mbf{C}_{AP_i}) \parallel \pi^{\auth}_{P_iB}(\mbf{K}^{\auth}_{P_iB} \parallel \mbf{C}_{P_iB})$. 
  
    From the properties of the pseudo-metric, we have%
    \begin{aeq}\label{eq:auth_2n_channel}
        d(\pi^g\mf{R}_g, \pi^s\mf{R}_s\sigma^{E^n}_{APB}) &\leq d(\{\pi^{\text{auth}}_{AP_iB}(\mbf{KC)}\}, \{\mbf{A}^{+}_{AP_iB}\sigma^E_{AP_iB}\})  \\
        & \leq \sum_{i=1}^n d(\pi^{\text{auth}}_{AP_iB}(\mbf{KC)}, \mbf{A}^{+}_{AP_iB}\sigma^E_{AP_iB}) \\
        & \leq 2n \epsilon',
    \end{aeq}%
    where we use \cref{eq:metric_serial_composition,eq:metric_parallel_composition} for the first inequality to remove common systems in $\pi^g\mf{R}_g$ and $\pi^s\mf{R}_s\sigma^{E^n}_{APB}$, \cref{thm:composability} for the second inequality and the security of the authentication protocol for the third inequality and the fact that there are $2n$ uses of the authentication protocol. 

    From \cref{thm:skeleton_security}, we also have a converter $\sigma^E$ such that%
    \begin{aeq}\label{eq:skeleton_secrecy}
        d(\pi^s\mf{R}_s, \mf{S}\sigma^E ) \leq \epsilon.
    \end{aeq}%
    Thus, we show that for the converter $\sigma'^E = \sigma^E \sigma^{E^n}_{APB}$, we have%
    \begin{aeq}
        &~ d(\pi^g\mf{R}_g, \mf{S}\sigma'^E) \\
        \leq &~ d(\pi^g\mf{R}_g, \pi^s\mf{R}_s\sigma^{E^n}_{APB}) + d(\pi^s\mf{R}_s\sigma^{E^n}_{APB}, \mf{S}\sigma^E\sigma^{E^n}_{APB}) \\
        \leq &~ d(\pi^g\mf{R}_g, \pi^s\mf{R}_s\sigma^{E^n}_{APB}) + d(\pi^s\mf{R}_s, \mf{S}\sigma^E)\\
        \leq &~ 2n\epsilon' + \epsilon,
    \end{aeq}%
    where we use the triangle inequality in the first inequality, \cref{eq:metric_serial_composition,eq:metric_parallel_composition} to drop the common system $\sigma^{E^n}_{APB}$ in the second inequality, and \cref{eq:auth_2n_channel,eq:skeleton_secrecy} in the third inequality.

    Combining those two conditions, we show that $\pi^g$ securely constructs the ideal resource $\mf{S}$ out of the resource $\mf{R}_g$ within $\max(\epsilon, \epsilon + 2n \epsilon')=\epsilon + 2n \epsilon'$.
\end{proof}

We then show the $\epsilon$-robustness of the general DSKE protocol.
\begin{theorem}[Robustness of a general DSKE protocol]\label{thm:robustness_general}
    When the upper bound on the number of compromised Security Hubs is no greater than $\min(n-k, k-1)$, a general DSKE protocol is $\epsilon$-robust with $\epsilon = \min({n \choose k} \frac{m+1}{|F|}, 1)$.
\end{theorem}
\begin{proof}
    This follows directly from Theorem \Cref{thm:robustness_skeleton}.
\end{proof}
 

==> text/removed/dske_preliminaries.tex <==
% \section{Composable Security of DSKE}
% \label{section:security}

% \subsection{Security Proof}
% Conceptually discuss security proof, and state (without direct proof in the paper) required theorems for the proof. Use same notation as A.2.

\section{Technical Preliminaries}
\label{sec:dske_preliminaries}

\subsection{Cryptographic primitives}

\subsubsection{Message validation (authentication)}

The following \cref{thm:hash_function_correctness} is a consequence of the hashing scheme being a Carter--Wegman universal hash function family \cite{wegman1981new}.  This polynomial function family is described by Bernstein \cite{Bernstein2007}.

\begin{theorem}\label{thm:hash_function_correctness} ~ \\
    Denote $\mbf{v} = (v_{1},...,v_{s})$ and $\mbf{v}^{*} = (v^{*}_{1},...,v^{*}_{s})$. \\
    Let $\Omega=F^2$ be a sample space with uniform probability. \\
    Let $h_{C,D}(\mbf{v})=D+\sum_{j=1}^{s}C^{j} v_{j}$ define a family of functions with random variables $(C,D)\in\Omega$ as selection parameters.
    Let $s\ne0$. Let $t\in F$ be given.
    Then, $\max_{t^{*},\mbf{v}^{*}\ne\mbf{v}} \Pr(t^{*}=h_{C,D}(\mbf{v}^{*})~|~t=h_{C,D}(\mbf{v})) = \min(\frac{s}{|F|},1)$.
\end{theorem}
\begin{proof}
	See \Cref{thm:message_correctness} in \Cref{app:hash_message}.
\end{proof}

Given a message $\mbf{v}$ together with a valid tag $t=h_{c,d}(\mbf{v})$ (with $(c,d)$ being described by the uniform random variables $C,D$), \cref{thm:hash_function_correctness} tells us that the maximal success probability for a forger to create a differing message $\mbf{v}^{*}$ and a new hash value $t^{*}$ such that these correspond (i.e., that $t^{*}=h_{C,D}(\mbf{v}^{*})$) is at most $\min(\frac{s}{|F|},1)$ when the message length $s$ is nonzero. This extends to $s=0$ due to the nonexistence of differing messages of that length.
In the other words, not knowing $(c,d)$ makes it highly improbable (for large $|F|$) for the forger to successfully substitute a tag and \textit{differing} message.

The theorem does not apply without a prior message. In the absence of a prior message, the probability that a forged message will be validated is $\frac{1}{|F|}$, which is independent of the length $s$.

\subsubsection{Secret confidentiality and validation}

Shamir introduced a secret sharing scheme that produces $n$ shares, any $k$ of which are sufficient to reconstruct the secret, but any $k-1$ of which give no information about the secret \cite{shamir1979share}. We state theorems here and leave proofs in \Cref{app:hash_secret}.

\begin{theorem}\label{thm:secret_confidentiality}
    In a Shamir secret sharing scheme with threshold $k$, the shared secret is independent of any subset of the shares of size $k-1$ or less.
\end{theorem}

\Cref{thm:secret_confidentiality} tells us that, under the constraint of access to only $k-1$ shares, a Shamir threshold-$(n,k)$ secret sharing scheme has perfectly secure confidentiality. 

\begin{theorem}\label{thm:secret_linearity}
    In a Shamir secret sharing scheme with threshold $k$, for any given set of $k$ shares, the secret is a linear combination of the shares.
\end{theorem}


\begin{theorem}\label{thm:hash_function_confidentiality}
    Denote $\mbf{Y}=(Y_{(1)},\dots,Y_{(m)})$. \\
    Let $\Omega=F^{3+m}$ be a sample space.
    Let $(C,D,E,\mbf{Y})\in\Omega$, with $D$ uniform and independent of $C,E$ and $\mbf{Y}$. \\
    Let $T=h'_{C,D,E}(\mbf{Y})=D+CE+\sum_{j=1}^{m}C^{j+1}Y_{(j)}$. \\
    Then $T$ is independent of $\mbf{Y}$.
\end{theorem}
Its proof is straightforward by using \Cref{lem:indepsum} in \Cref{app:hash_secret}. \Cref{thm:hash_function_confidentiality} tells us that no information is obtained from the tag ($o^A$ as $T$) about the secret ($S^A$ as $\mbf{Y}$).  Thus, given the perfectly secure confidentiality provided by a Shamir secret sharing scheme for up to $k-1$ shares being known, publishing the tag does not impact this confidentiality.

Given a Shamir secret sharing scheme, the resulting secret is malleable: a modification of any share will modify the reconstructed secret in a known way, in the same way that modifying the ciphertext of one-time-pad encryption modifies the decrypted plaintext.  Normally, a message authentication code would be employed to allow detection of such a change, but this needs a shared key to implement.  Transmitting a validation key via the same secret sharing scheme violates the normal premise for authentication: that the validation key is assured to be the same at both sides.  \Cref{thm:secret_validation} gives us a way to transmit such a key using the same (malleable) secret sharing scheme while providing authenticity, under the same premise that the secret sharing scheme already has.  We believe that this is a novel construction\footnote{A related objective is presented in \cite{ostrev2019composable}.}.

\begin{theorem}\label{thm:secret_validation}
    Denote $\mbf{y}=(y_{(1)},\dots,y_{(m)})$ and $\mbf{y}'=(y'_{(1)},\dots,y'_{(m)})$.
    Let $\Omega=F^3$ be a sample space with uniform probability.
    Let $h'_{C,D,E}(\mbf{y})=D+CE+\sum_{j=1}^{m}C^{j+1}y_{(j)}$ define a family of hash functions with random variables $(C,D,E)\in\Omega$ as selection parameters. Let $m\ne0.$
    Then, $\max_{t',c',d',e',\mbf{y}'\ne\mbf{y}} \Pr(t+t'=h'_{C+c',D+d',E+e'}(\mbf{y}+\mbf{y}')~|~t=h'_{C,D,E}(\mbf{y}))\le\min(\frac{m+1}{|F|},1)$.
\end{theorem}

\Cref{thm:secret_validation} gives us an upper bound on the probability of validating a secret with a nontrivial alteration, with three confidential uniform elements and the alteration constrained to \textit{addition} of a vector to $(C,D,E,\mbf{y})$. The premise for the theorem is assured by the secret sharing scheme. There are $n\choose k$ subsets of $k$ shares and hence reconstructions, but a probability is upper-bounded at $1$, giving an upper bound on the probability of any of the ${n\choose k}$ reconstructed secret candidates passing the validation of $\epsilon\le\min({n\choose k}\frac{m+1}{|F|},1)$.

Combining \Cref{thm:secret_confidentiality,thm:secret_linearity,thm:hash_function_confidentiality,thm:secret_validation} leads to the following result:

The $(n,k)$-Shamir secret sharing scheme and a polynomial validation code for transmitting $3+m$ elements of the same finite field $F$, where the first 3 elements are uniform, of which the first $3$ are consumed as $u^A$ and the remaining $m$ elements are $S^A$, has
\begin{itemize}
    \setlength\itemsep{0em}
    \item $\epsilon$-secure correctness with $\epsilon\le\min({n\choose k}\frac{m+1}{|F|},1)$
    \item perfectly secure confidentiality
\end{itemize}
against a computationally unbounded adversary who can access and modify up to $k-1$ shares and block but not access or modify any of the remaining shares.

This leverages the secrecy provided by the sharing scheme to deliver the key used for secure validation of the secret that is simultaneously delivered.  This is novel in the sense that it ensures correctness (authentication) in addition to retaining the confidentially of the secret sharing scheme without imposing additional security requirements, i.e., it assumes only that no more than $k-1$ of the shares are compromised, as with the sharing scheme, whereas normally the key for validation would be assumed to be pre-shared.

\subsection{Composability and constructive cryptography}\label{subsec:abstrac_crypto}

As a cryptographic protocol is often combined with many other protocols, it is important to prove the security of the protocol in a composable security framework. The composability result in such a framework asserts that in analyzing the security of a complex protocol, one can simply decompose it into various subprotocols and analyze the security of each. Provided that each real subsystem constructed by a subprotocol is close to an ideal subsystem within some $\epsilon$, which is quantified by some distance measure (a pseudo-metric in abstract cryptography), the real system constructed from the combined protocol will then be close to the combined ideal system. The sum of the $\epsilon$-values for the subprotocols gives an $\epsilon$-value for the combined protocol.

The abstract cryptography framework \cite{MaurerRenner2011} uses a top-down approach. In this framework, one states the definitions and proves the security from the highest possible level of abstraction and proceeds downwards. When one deals with a specific instantiation of an abstract system in a lower level, as long as the lower level system satisfies the properties required in the higher-level proof, the composed protocol is secure. The constructive cryptography \cite{Maurer2011} is an application of the abstract cryptography framework to defining classical cryptographic primitives in a constructive way. In this framework, one specifies the resources that are used by a protocol, their required properties and some desired functionalities of an ideal system. If a protocol constructs the ideal system from the given resources, then it is secure. A protocol that is secure in this sense is also universally composable secure. We briefly review the composable security definition in the constructive cryptography framework below and refer to \cite{Maurer2011} for further details.

% reword last sentence of para. 3
% Need to introduce theorem in a few sentences
 
\begin{definition}\label{def:composable_security}
    Let $\mf{R}$ and $\mf{S}$ be resources with the interface label set $\mc{I} =\{A, B, E\}$. Let $d$ be a pseudo-metric. We say that a protocol $\pi = (\pi^A, \pi^B)$ securely constructs $\mf{S}$ out of $\mf{R}$ within $\epsilon$ if the following conditions hold:
    \begin{enumerate}[label=(\roman*)]
        \item For converters $\alpha^E$ and $\gamma^E$ that emulate an honest behaviour at the $E$-interface of each system and block any distinguisher from the access of $E$-interface of each system,%
        \begin{aeq}
            d(\pi\mf{R}\alpha^E, \mf{S}\gamma^E) \leq \epsilon.
        \end{aeq}
        \item There exists a converter $\sigma^E$ such that%
        \begin{aeq}
            d(\pi \mf{R}, \mf{S}\sigma^E) \leq \epsilon.
        \end{aeq}%
    \end{enumerate}
    We use the construction notation $\mf{R} \xrightarrow{(\pi, \epsilon)} \mf{S}$ for this case.
\end{definition}

% replace the composability thoerem with [21, theorem 1]

\subsection{Threat Model}
\label{subsec:threat_model}

A collection of adversarial entities can include a coalition of end users other than Alice and Bob, eavesdroppers, and a subset of the Security Hubs. A compromised Security Hub may deviate from the protocol. No limits are placed on compromised hubs, but they cannot access or modify any confidential information held by other parties. This set of adversaries may collude to attempt to compromise the objective of the protocol between Alice and Bob. We call this collection of adversarial entities \textit{Eve}. 

As a robustness analysis of a protocol is concerned with an honest implementation of the protocol, which is a modified threat model from that of the correctness and confidentiality (i.e. \Cref{subsec:ideal_system}) analysis, we call Eve's behaviour \textit{passive Eve}: Eve is passive on all communication links, that is, she is allowed to listen to all the communications except for the initial sharing of tables by honest Security Hubs but she does not tamper; she is still given the ability to fully control compromised Security Hubs. When Eve is passive, we show that the DSKE protocol completes (i.e., does not abort) with a high probability.

\subsection{Assumptions}
\label{subsec:assumptions}

We list assumptions used in our security proof:
\begin{enumerate}[label = \roman*)]
    \item The pre-shared random data (PSRD) are securely delivered by all uncompromised Security Hubs to both Alice and Bob. By \textit{securely delivered}, we mean ensured confidentiality, integrity and proper identity verification through secure channels between Security Hubs and clients.\footnote{PSRD can be delivered by physically shipping a secure data storage device or via QKD links.}.
    \item The two users, Alice and Bob, are both honest.
    \item A number of the Security Hubs might be compromised, and this number has a known upper bound. 
    \item For the robustness analysis, a number of the involved Security Hubs might malfunction, either due to unavailability, communication failure\footnote{This type of malfunction includes the possibility that a communication link incorrectly provides the originating identity to the receiver.}, or compromise, and this number has a known upper bound. This is incorporated with the assumption that Eve is passive on the communication links.
\end{enumerate}


==> text/removed/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Pre-shared keys have been used in cryptography for thousands of years. The famous "Caesar" shift cipher, one of the first uses of a pre-shared key, involves shifting the letters in a message by a constant amount in the alphabet. As the technology evolved, to encompass random mappings of letters in the alphabet, employing keywords to shift messages, and configuring initial positions of electro-mechanical encryption devices, so too has the field of cryptographic attacks \cite{Kotas2000ABH}. 

Currently, pre-shared keys (PSKs) are widely used in commercial applications, such as sensor networks, banking, and government, as they are a simplistic encryption solution that offers high security. A sensor network is a distributed network of small, low-cost devices (referred to as nodes) equipped with sensors that collect and transmit data about the physical environment for various applications\cite{Chan2004}. Depending on the use case, information travelling between nodes can be very confidential, therefore requiring high security. Numerous methods of node-to-node encryption exist, including asymmetric encryption, which is computationally expensive and unprovably secure, a network-wide PSK, which can lead to a network-wide breach if a single node is compromised, and pairwise-shared keys, which while being the most secure option, is difficult to scale in a large network due to onboarding costs increasing with network size and each resource-constrained node being required to store $n-1$ keys, where $n$ is the total number of nodes \cite{Chan2004}. The addition of a new node to the network would require updating all $n$ nodes' key rings\cite{Chan2004}. For Banking, the American National Standards Institute (ANSI) for Financial Services' symmetric key management standards (ANSI X9.69 Standard) proposes a protocol for dynamically generated PSKs between clients in a network, called Constructive Key Management (CKM). It involves sending information between network clients in the form of attributes, which are used to reconstruct a symmetric key\cite{ansi2023}. Dynamically generating keys pushes PSKs forward, as this algorithm reduces the storage need, although, single-point-of-failure risks arise, as a breach of the CKM could lead to an adversary obtaining all attributes and deducing any key in the network. Regarding government communications, they may opt for a highly secure protocol, like High Assurance Internet Protocol Encryptor (HAIPE), to transmit confidential information. HAIPE is a layer 3 encryption device based on IPsec with additional restrictions and enhancements. Like many other top secret communication protocols, HAIPE requires PSKs\cite{cnssi2022}.

In order to have a robust PSK system, keys must have sufficient length and randomness to protect against brute-force attacks, keys should be rotated in regular intervals to mitigate excessive information about the key being leaked, key management entities must have advanced security measures to prevent the leakage of information, and keys must be securely distributed prior to communication. Often, the greatest challenge of a PSK system lies in the distribution of PSKs and preventing the leakage of information by key management entities. If every user in a network were to share a unique key between each other, the cost of onboarding a new user would increase as it is proportional to the number of users in the network, as briefly mentioned in our discussion of pairwise-shared keys in a sensor network\cite{Chan2004}. Not to mention, as the distance between two users increases, it becomes more difficult to securely transport the key. Additionally, the breach of centralized entities in a PSK network, such as the CKM system discussed in banking\cite{ansi2023}, could prove catastrophic to the entire network. Essentially, PSK systems suffer from their lack of scalability, forcing large cryptosystems to resort to cryptographic techniques such as public key cryptography. 

We fill this big gap by proposing a new protocol, called Distributed Symmetric Key Exchange (DSKE), which is based on secret sharing. The basis on secret sharing allows for distributed trust among multiple semi-trusted entities, alleviating single-point-of-failure risks. DSKE's client onboarding process is independent of the size of the network, making a PSK system scalable on a worldwide level. In order to ensure that DSKE remains secure against future unknown cryptographic attacks, we provide a composable proof of DSKE's information-theoretic security against a computationally unbounded eavesdropper that can observe all communication, form a collusion between clients, and control under a threshold number of Security Hubs. To showcase DSKE's current integration abilities, we conduct several experiments, including setting up a Layer 3 VPN between clients with DSKE PSKs, using QKD to deliver pre-shared random data (PSRD), using Key Management Entities (KMEs) to interface with numerous encryption devices, and having end-to-end encrypted conversations between mobile phone DSKE clients.

The remainder of this paper is organized as follows. We discuss the need for quantum-safe cryptography, and the current types of solutions today in \Cref{sec:postquantum}. In \Cref{sec:dske}, we discuss the details of the DSKE protocol. We then introduce technical preliminaries in \Cref{sec:dske_preliminaries}, and prove the Security of the protocol in \Cref{sec:dske_security}. We review the current implementations of DSKE in \Cref{sec:implementation}. We analyze the future of DSKE and conclude in \Cref{sec:discussionconclusion}.

==> text/removed/problems_pqc.tex <==
\section{Current Quantum-Safe Solutions}
\label{sec:postquantum}

As society has apprehensions about the security of conventional cryptographic methods, in particular, our vast Public Key Infrastructure systems, which secures an enormous amount of communication on the internet, a transition towards quantum-safe solutions has begun. Innovation has taken off in three main pillars which underpin the realm of quantum-safe cryptography: (the redesign of) Public Key Infrastructure (PKI) often referred to as Post-Quantum Cryptography (PQC), Quantum Key Distribution (QKD), and Pre-Shared Key (PSK) cryptography.

PKI is based on asymmetric encryption, using mathematically related keys (public and private) to encrypt and decrypt data. Popular conventional asymmetric systems, such as RSA (Rivest-Shamir-Adleman), ECC (Elliptic curve cryptography), and DH (Diffie-Hellman) key exchange are thought to be under threat by quantum computers. Concretely, RSA and DH algorithms can be cracked by Shor's algorithm \cite{Shor_1997}, and ECC by Discrete Log algorithms \cite{proos2004shors}. Due to PKI being software based, highly scalable, and deeply ingrained in modern society, there is pressure to develop quantum resistant PKI algorithms, referred to as PQC. Even with new algorithms, PQC will continue to suffer from being computationally expensive, as well as being unprovably safe against quantum attacks. This inability to prove PQC's security can cause a quantum "cat-and-mouse" game of code makers and code breakers, where data is in a state of perpetual risk. 

QKD is a key distribution technique which allows two parties to obtain a shared key for use in symmetric cryptography. It is based on the no-cloning theorem in quantum mechanics, which states that one cannot copy an arbitrary unknown quantum state into a blank state without change to the original state. QKD is provably secure, and eavesdroppers can always be identified during key exchange. The fact that QKD is unconditionally secure makes it a very attractive solution. However, QKD has limited range\footnote{The maximum theoretical length of a TF-QKD link (one of the best QKD methods in terms of the distance-rate tradeoff) that supports relatively high key rates ($\sim$ 100 bits/second) is only about about 400 km\cite{Lucamarini_Yuan_Dynes_Shields_2018}.}, key rate ability, and requires dedicated optical fibers and expensive appliances for each communication link. Even when limited range is circumvented by using relay devices such as quantum repeaters, the cost of the single link increases significantly. To connect pairs of clients in a large network, $\frac{n(n-1)}{2}$ QKD links are required, where $n$ is the number of clients, and the cost of onboarding a new client is proportional to the number of clients in the network. In short, current QKD technology alone is not scalable. 

PSK, being a form of symmetric cryptography, is the oldest cryptographic technique discussed here. Data is encrypted and decrypted by using a secret key that both communication parties share beforehand. PSK is provably secure when the pre-sharing of keys is done privately. However, because an individual client is often unable to manually distribute a key to other parties in the network, they require a trusted key distribution center. From here, key distribution would occur through a secure channel\footnote{Often, this takes place over a physical shipment in a Pre-Shared Key Module (PSKM).} to each client in the network. Keys would need to pre-shared amongst every pair of clients in the network, requiring $\frac{n(n-1)}{2}$ PSKs, which also need to be cycled to maintain security. This causes issues in trust and scalability. The key distribution center holds information about every single key in the network, making it an attractive target to would-be eavesdroppers. Additionally, physical key shipments can be difficult to make across long distances. This makes traditional PSK unscalable.

Often, multiple layers of encryption are performed to increase security and seamlessness of the integration of new cryptographic techniques. The combination of different encryption methods can cover up individual weaknesses, such as combining PQC's versatility with PSK's provable security. As for the integration of new techniques, it is often easier to supplement existing encryption methods without having to replace the system. An example of this would be supplying an additional PSK alongside an existing PQC algorithm, instead of removing the PQC system and building a new PSK system.

With unprovable security of PQC, and the impact of failure of cryptographic systems being so large, there is much scientific interest in understanding provably-secure alternatives to PQC \cite{quantum2030}. Even though new asymmetric algorithms are being developed, it is always hard to predict how it will perform against attacks. For example, the Rainbow signature scheme, part of the NIST Post-Quantum Cryptography Standardization project, was thought by many to be both classical and quantum computer resistant, but ended up being cracked in 53 hours by a laptop with a single-core CPU \cite{10.1007/978-3-031-15979-4_16}. This begs for a layer of provably-reliable encryption, and despite its barriers, PSKs are an attractive solution. In 2022, the NSA stated that PSKs should be used instead of or in addition to asymmetric algorithms, and as the magnitude of the quantum threat becomes clearer, more begin to agree \cite{threat_quantum_2022, csfc2022, rfc8784}.

PSKs are indifferent towards the exact encryption algorithm performed with the PSK, such as an AES mode \cite{aesmodes}, or a ChaCha20 algorithm \cite{chacha}. The crux is the key distribution process. As previously mentioned, this often takes place over physical delivery, usually coordinated by a centralized key distribution center. We conceptualize a PSK network where every pair of clients share a PSK, managed by the central key distribution center. With each new client, a new PSK must be generated and shipped to every client in the network. This makes for $n-1$ (including the new client in the total, $n$) new keys, and $n$ physical deliveries. As the network gets larger, it becomes a logistical nightmare to coordinate, and is unreasonable on a global scale. This is a big reason why PKI and PQC are so much more common today. Next, this key distribution center stores the information to decrypt all communication in the network, making it a big target for hackers. Even if a lot of attention was put into assuring the security of the key distribution center, the risk it holds is too much, especially in worldwide networks.
